Strong-field Coherent Control of Isolated Attosecond Pulse Generation

Attosecond science promises to reveal the most fundamental electronic dynamics occurring in matter and it can develop further by meeting two linked technological goals related to high-order harmonic sources: higher photon flux (permitting to measure low cross-section processes) and improved spectral tunability (allowing selectivity in addressing specific electronic transitions). New developments come through parametric waveform synthesis, which provides control over the shape of high-energy electric field transients, enabling the creation of highly-tunable isolated attosecond pulses via high-harmonic generation. Here we show that central energy, spectral bandwidth/shape and temporal duration of the attosecond pulses can be controlled by shaping the laser pulse waveform via two key parameters: the relative-phase between two halves of the multi-octave spanning optical spectrum, and the overall carrier-envelope phase. These results not only promise to expand the experimental possibilities in attosecond science, but also demonstrate coherent strong-field control of free-electron trajectories using tailored optical waveforms.

==> new_bib.tex <==
%\normalem % removes underlines caused by ulem command
%\bibliography{NatPhotBib}
\newpage
\begin{thebibliography}{99}

\bibitem{Corkum2007} Corkum, P. B. \& Krausz, F. Attosecond science. \textit{Nat. Phys.} \textbf{3}, 381–387 (2007).

\bibitem{Calegari2014} Calegari, F. \textit{et al.} Ultrafast electron dynamics in phenylalanine initiated by attosecond pulses. \textit{Science} \textbf{346}, 336–339 (2014).

\bibitem{Hassan2016} Hassan, M. T. \textit{et al.} Optical attosecond pulses and tracking the nonlinear response of bound electrons. \textit{Nature} \textbf{530}, 66–70 (2016).

\bibitem{Beaulieu2018} Beaulieu, S. \textit{et al.} Attosecond-resolved photoionization of chiral molecules. \textit{Science} \textbf{358}, 1288–1294 (2017).

\bibitem{Levin2015} Levin, L. \textit{et al.} Coherent Control of Bond Making. \textit{Phys. Rev. Lett.} \textbf{114}, 233003 (2015).

\bibitem{Golubev2015} Golubev, N. V. \& Kuleff, A. I. Control of charge migration in molecules by ultrashort laser pulses. \textit{Phys. Rev. A} \textbf{91}, 051401 (2015).

\bibitem{Wimmer2014} Wimmer, L. \textit{et al.} Terahertz control of nanotip photoemission. \textit{Nat. Phys.} \textbf{10}, 432–436 (2014).

\bibitem{Wang2016} Wang, W. T. \textit{et al.} High-Brightness High-Energy Electron Beams from a Laser Wakefield Accelerator via Energy Chirp Control. \textit{Phys. Rev. Lett.} \textbf{117}, 124801 (2016).

\bibitem{Kim2017} Kim, H. T. \textit{et al.} Stable multi-GeV electron accelerator driven by waveform-controlled PW laser pulses. \textit{Sci. Rep.} \textbf{7}, 10203 (2017).

\bibitem{Guenot2017} Gu{\'{e}}not, D. \textit{et al.} Relativistic electron beams driven by kHz single-cycle light pulses. \textit{Nat. Photon.} \textbf{11}, 293–296 (2017).

\bibitem{Zhang2018} Zhang, D. \textit{et al.} Segmented terahertz electron accelerator and manipulator (STEAM). \textit{Nat. Phot.} \textbf{12}, 336–342 (2018).

\bibitem{Sansone2006} Sansone, G. \textit{et al.} Isolated Single-Cycle Attosecond Pulses. \textit{Science} \textbf{314}, 443–446 (2006).

\bibitem{Gaumnitz2017} Gaumnitz, T. \textit{et al.} Streaking of 43-attosecond soft-X-ray pulses generated by a passively CEP-stable mid-infrared driver. \textit{Opt. Express} \textbf{25}, 27506–27518 (2017).

\bibitem{Chang2007} Chang, Z. Controlling attosecond pulse generation with a double optical gating. \textit{Phys. Rev. A} \textbf{76}, 051403 (2007).

\bibitem{Abel2009} Abel, M. J. \textit{et al.} Isolated attosecond pulses from ionization gating of high-harmonic emission. \textit{Chem. Phys.} \textbf{366}, 9–14 (2009).

\bibitem{Hammond2016} Hammond, T. J., Brown, G. G., Kim, K. T., Villeneuve, D. M. \& Corkum, P. B. Attosecond pulses measured from the attosecond lighthouse. \textit{Nat. Photon.} \textbf{10}, 171–175 (2016).

\bibitem{Chipperfield2009} Chipperfield, L. E., Robinson, J. S., Tisch, J. W. G. \& Marangos, J. P. Ideal waveform to generate the maximum possible electron recollision energy for any given oscillation period. \textit{Phys. Rev. Lett.} \textbf{102}, 063003 (2009).

\bibitem{Wu2010} Wu, J., Zhang, G.-T., Xia, C.-L. \& Liu, X.-S. Control of the high-order harmonics cutoff and attosecond pulse generation through the combination of a chirped fundamental laser and a subharmonic laser field. \textit{Phys. Rev. A} \textbf{82}, 013411 (2010).

\bibitem{Jin2014} Jin, C., Wang, G., Wei, H., Le, A. T. \& Lin, C. D. Waveforms for optimal sub-keV high-order harmonics with synthesized two- or three-colour laser fields. \textit{Nat. Commun.} \textbf{5}, 4003 (2014).

\bibitem{Chou2015} Chou, Y., Li, P.-C., Ho, T.-S. \& Chu, S.-I. Optimal control of high-order harmonics for the generation of an isolated ultrashort attosecond pulse with two-color midinfrared laser fields. \textit{Phys. Rev. A} \textbf{91}, 063408 (2015).

\bibitem{Tate2007} Tate, J. \textit{et al.} Scaling of Wave-Packet Dynamics in an Intense Midinfrared Field. \textit{Phys. Rev. Lett.} \textbf{98}, 013901 (2007).

\bibitem{Heyl2017} Heyl, C. M., Arnold, C. L., Couairon, A. \& L’Huillier, A. Introduction to macroscopic power scaling principles for high-order harmonic generation. \textit{J. Phys. B} \textbf{50}, 013001 (2017).

\bibitem{Popmintchev2009} Popmintchev, T. \textit{et al.} Phase matching of high harmonic generation in the soft and hard X-ray regions of the spectrum. \textit{Proc. Natl. Acad. Sci. USA} \textbf{106}, 10516–10521 (2009).

\bibitem{Teichmann2016} Teichmann, S. M., Silva, F., Cousin, S. L., Hemmer, M. \& Biegert, J. 0.5-keV Soft X-ray attosecond continua. \textit{Nat. Comm.} \textbf{7}, 11493 (2016).

\bibitem{Wirth2011} Wirth, A. \textit{et al.} Synthesized light transients. \textit{Science} \textbf{334}, 195–200 (2011).

\bibitem{Harth2012} Harth, A. \textit{et al.} Two-color pumped OPCPA system emitting spectra spanning 1.5 octaves from VIS to NIR. \textit{Opt. Express} \textbf{20}, 3076–3081 (2012).

\bibitem{Schmidt2014} Schmidt, B. E. \textit{et al.} Frequency domain optical parametric amplification. \textit{Nat. Comm.} \textbf{5}, 3643 (2014).

\bibitem{Huang2011} Huang, S.-W. \textit{et al.} High-energy pulse synthesis with sub-cycle waveform control for strong-field physics. \textit{Nat. Photon.} \textbf{5}, 475–479 (2011).

\bibitem{Manzoni2012} Manzoni, C. \textit{et al.} Coherent synthesis of ultra-broadband optical parametric amplifiers. \textit{Opt.
Lett.} \textbf{37}, 1880–1882 (2012).

\bibitem{Fattahi2014} Fattahi, H. \textit{et al.} Third-generation femtosecond technology. \textit{Optica} \textbf{1}, 45–63 (2014).

\bibitem{Liang2017} Liang, H. \textit{et al.} High-energy mid-infrared sub-cycle pulse synthesis from a parametric amplifier. \textit{Nat. Commun.} \textbf{8}, 141 (2017).

\bibitem{Brida2010} Brida, D. \textit{et al.} Few-optical-cycle pulses tunable from the visible to the mid-infrared by optical parametric amplifiers. \textit{J. Opt.} \textbf{12}, 013001 (2010).

\bibitem{Baltuska2002} Baltu{\v{s}}ka, A., Fuji, T. \& Kobayashi, T. Controlling the Carrier-Envelope Phase of Ultrashort Light Pulses with Optical Parametric Amplifiers. \textit{Phys. Rev. Lett.} \textbf{88}, 133901 (2002).

\bibitem{Manzoni2016} Manzoni, C. \& Cerullo, G. Design criteria for ultrafast optical parametric amplifiers. \textit{J. Opt.} \textbf{18}, 103501 (2016).

\bibitem{Rossi2018} Rossi, G. M. \textit{et al.} CEP dependence of signal and idler upon pump-seed synchronization in optical parametric amplifiers. \textit{Opt. Lett.} \textbf{43}, 178–181 (2018).

\bibitem{Brida2008} Brida, D. \textit{et al.} Sub-two-cycle light pulses at 1.6 $\mu$m from an optical parametric amplifier. \textit{Opt. Lett.} \textbf{33}, 741–743 (2008).

\bibitem{Birge2006} Birge, J. R., Ell, R. \& K{\"{a}}rtner, F. X. Two-dimensional spectral shearing interferometry for few-cycle pulse characterization. \textit{Opt. Lett.} \textbf{31}, 2063–2065 (2006).

\bibitem{Mucke2015} M{\"{u}}cke, O. D. \textit{et al.} Toward Waveform Nonlinear Optics Using Multimillijoule Sub-Cycle Waveform Synthesizers. \textit{J. Sel. Top. Quantum Electron.} \textbf{21}, 8700712 (2015).

\bibitem{Chia2014} Chia, S.-H. \textit{et al.} Two-octave-spanning dispersion-controlled precision optics for sub-opticalcycle waveform synthesizers. \textit{Optica} \textbf{1}, 315–322 (2014).

\bibitem{Mairesse2005} Mairesse, Y. \& Qu{\'{e}}r{\'{e}}, F. Frequency-resolved optical gating for complete reconstruction of attosecond bursts. \textit{Phys. Rev. A} \textbf{71}, 011401 (2005).

\bibitem{Keathley2016} Keathley, P. D., Bhardwaj, S., Moses, J., Laurent, G. \& K{\"{a}}rtner, F. X. Volkov transform generalized projection algorithm for attosecond pulse characterization. \textit{New J. Phys.} \textbf{18}, 073009 (2016).

\bibitem{Kim2013} Kim, K. T. \textit{et al.} Petahertz optical oscilloscope. \textit{Nat. Photon.} \textbf{7}, 958–962 (2013).

\bibitem{Wyatt2017} Wyatt, A. S. \textit{et al.} Attosecond sampling of arbitrary optical waveforms. \textit{Optica} \textbf{3}, 303–310 (2016).

\bibitem{Gagnon2011} Gagnon, J. \& Yakovlev, V. S. The direct evaluation of attosecond chirp from a streaking measurement. \textit{Appl. Phys. B} \textbf{103}, 303–309 (2011).

\bibitem{Gustas2018} Gustas, D. \textit{et al.} High-charge relativistic electron bunches from a kHz laser-plasma accelerator. \textit{Phys. Rev. Accel. Beams} \textbf{21}, 013401 (2018).

\bibitem{Lifschitz2012} Lifschitz, A. F. \& Malka, V. Optical phase effects in electron wakefield acceleration using few-cycle laser pulses. \textit{New J. Phys.} \textbf{14}, 053045 (2012).

\bibitem{Putnam2017} Putnam, W. P., Hobbs, R. G., Keathley, P. D., Berggren, K. K. \& K{\"{a}}rtner, F. X. Optical-field-controlled photoemission from plasmonic nanoparticles. \textit{Nat. Phys.} \textbf{13}, 335–339 (2017).

\bibitem{Liu2012} Liu, K., Zhang, Q. \& Lu, P. Enhancing electron localization in molecular dissociation by two-color mid- and near-infrared laser fields. \textit{Phys. Rev. A} \textbf{86}, 033410 (2012).

\bibitem{Nicoletti2016} Nicoletti, D. \& Cavalleri, A. Nonlinear lightmatter interaction at terahertz frequencies. \textit{Adv. Opt. Photonics} \textbf{8}, 401–464 (2016).


\end{thebibliography}
